Aspects of Quantum Entanglement and Indistinguishability

This thesis investigates the entanglement of distinguishable and indistinguishable particles, introducing a new error model for Hardy's test, experimentally verified using superconducting qubits. We address challenges in implementing quantum protocols based on this test and propose potential solutions and present two performance measures for qubits in superconducting quantum computers. We demonstrate that if quantum particles can create hyper-hybrid entangled states and achieve unit fidelity quantum teleportation, arbitrary state cloning is possible. This leads to two no-go theorems: hyper-hybrid entangled states cannot be formed with distinguishable particles, and unit fidelity quantum teleportation is unattainable with indistinguishable particles. These results establish unique correlations for each particle type, creating a clear distinction between the two domains. We also show that hyper-hybrid entangled states can be formed with indistinguishable fermions and generalize this for both fermions and bosons. We develop a generalized DoF trace-out rule applicable to single or multiple degrees of freedom for both types of particles. This framework allows us to derive expressions for teleportation fidelity and singlet fraction, establishing an upper bound for the generalized singlet fraction. We present an optical circuit that generates entanglement in distinguishable particles. Using our trace-out rule, we show that for two indistinguishable particles with multiple DoFs, the monogamy of entanglement can be maximally violated. We assert that indistinguishability is essential for this violation in qubit systems. For three indistinguishable particles, we confirm that monogamy is upheld using squared concurrence. Finally, we propose a novel entanglement swapping protocol involving two indistinguishable particles, enhancing quantum networks and quantum repeaters.

==> Certificate/Certi.tex <==
\begin{center}
\textbf{{\Large CERTIFICATE FROM SUPERVISOR}}
\end{center}

This is to certify that the thesis entitled \textbf{Aspects of Quantum Entanglement and Indistinguishability} submitted by \textbf{Mr. Soumya Das}, a student of Cryptology and Security Research Unit of the Ph.D. program of Indian Statistical Institute Kolkata, is based upon his
research work under my supervision. This is also to certify that neither the thesis as a whole
nor as a part of it has been submitted for any degree/diploma or any other academic award
anywhere before. In my opinion, the thesis fulfills the requirement for the award of the de-
gree of Doctor of Philosophy.

\begin{flushleft}
\begin{figure}[h!]
\includegraphics[width=6cm]{./Certificate/Goutam_paul.jpeg} 
\end{figure}


\textbf{Dr. Goutam Paul} \\
Associate Professor\\
Cryptology and Security Research Unit\\
R. C. Bose Centre for Cryptology and Security\\
Indian Statistical Institute\\
Kolkata 700108, West Bengal, India\\
\end{flushleft}

==> Chap4/chap4_HHES_highlighted.tex <==
\chapter{Quantum teleportation and hyper-hybrid entangled state}\label{Chap4}
In this Section, we show that some properties and applications of distinguishable and indistinguishable entanglement. First, we show that hyper-hybrid entanglement can exists for two indistinguishable fermions. Then I have generalized it for both bosons and fermions. Next, we prove that \textit{quantum particles (either distinguishable or indistinguishable) can simultaneously produce and perform hyper hybrid entangled state and unit fidelity quantum teleportation respectively then using that cloning of any arbitrary quantum state is possible}. As the no-cloning theorem cannot be violated using in quantum theory, the logical conclusion from this statement can be written in the form of two no-go theorems; (i) \textit{no-hyper hybrid entangled state for distinguishable particles} and (ii) \textit{no-unit fidelity quantum teleportation for indistinguishable particles}. Finally we show the overall picture of the properties and applications of distinguishable and indistinguishable particles.  

 This chapter is based on the work in~\cite{Das20}.



\section{Hyper-hybrid entangled state for two indistinguishable fermions} \label{HHESfermions} 
{\color{blue} Yurke and Stolar~\cite{Y&S92PRA,Y&S92PRL} had proposed an optical circuit to generate quantum entanglement between the same DoFs of two identical particles (bosons and fermions) from initially separated independent sources. Some recent
experiments realizing entanglement between the same DoFs of identical particles whose degree of spatial indistinguishability can be arbitrarily harnessed~\cite{Sun2020,Sun2022,Wang2021,Wang2022}. The experiments are realized not only with photons but also simulating fermions.
Recently, the above method has been extended by Li \textit{et al.}~\cite{HHNL} to generate hyper-hybrid entangled state between two independent bosons among their internal (e.g., spin) DoFs, external (e.g., momentum) DoFs, and across. We show that their circuit can also be used for independent fermions obeying the Pauli exclusion principle~\cite{Pauli25}, albeit with different detection probabilities.}

For fermions, the second quantization formulation deals with fermionic creation operators $f_{i,\textbf{p}}$ with $\ket{i,\textbf{p}}=f^{\dagger}_{i,\textbf{p}}\ket{0}$, where $\ket{0}$ is the vacuum and $\ket{i,\textbf{p}}$ describes a particle with spin $\ket{i}$ and momentum $\textbf{p}$. These operators satisfy the canonical anticommutation relations:
\begin{equation} 
\left\lbrace f_{i,\textbf{p}_{i}}, f_{j,\textbf{p}_{j}}\right\rbrace = 0, \hspace{0.2cm} \left\lbrace f_{i,\textbf{p}_{i}}, f^{\dagger}_{j,\textbf{p}_{j}}\right\rbrace = \delta\left( \textbf{p}_{i}-\textbf{p}_{j}\right)\delta_{ij}.
\end{equation}

Analysis of the circuit of Li \textit{et al.}~\cite[Fig. 2]{HHNL} as shown in Fig.~\ref{fig:Lietal} for fermions involves an array of hybrid beam splitters (HBSs)~\cite[Fig. 3]{HHNL}; phase shifter; four orthogonal external modes $L$, $D$, $R$, and $U$; and two orthogonal internal modes $\uparrow$ and $\downarrow$. Here, particles exiting through the modes $L$ and $D$ are received by Alice (A), who can control the phases $\phi_{L}$ and $\phi_{D}$, whereas particles exiting through the modes $R$ and $U$  are received by Bob (B), who can control the phases $\phi_{R}$ and $\phi_{U}$. 

In this circuit~\cite[Fig. 2]{HHNL} as shown in Fig.~\ref{fig:Lietal}, two particles, each with spin $\ket{\downarrow}$, enter the setup in the mode $R$ and $L$ for Alice and Bob, respectively. The initial state of the two particles is $\ket{\Psi_{0}}=f^{\dagger}_{\downarrow,R} f^{\dagger}_{\downarrow,L}\ket{0}$. Now, the particles are sent to the HBS such that one output port of the HBS is sent to the other party ($R$ or $L$) and the other port remains locally accessible ($D$ or $U$). Next, each party applies path-dependent phase shifts. Lastly, the output of the local mode and that received from the other party are mixed with the HBS and then the measurement is performed in either  external or internal modes. The final state can be written as
\begin{equation} \label{Final_state_fermion}
\begin{aligned}
&\ket{\Psi}=\frac{1}{4} \left[ e^{i\phi_{R}}\left( f^{\dagger}_{\downarrow,R}+if^{\dagger}_{\uparrow,U}\right) +ie^{i\phi_{D}} \left( f^{\dagger}_{\uparrow,D} + i f^{\dagger}_{\downarrow,L}\right)  \right] \\
& \otimes \left[ e^{i\phi_{L}} \left( f^{\dagger}_{\downarrow,L}+if^{\dagger}_{\uparrow,D}\right)  + i e^{i\phi_{U}}\left( f^{\dagger}_{\uparrow,U}+if^{\dagger}_{\downarrow,R}\right) \right] \ket{0}.
\end{aligned}
\end{equation} 
Alice and Bob can perform coincidence measurements both in external DoFs or both in internal DoFs or with one party in the internal DoF and the other in the external DoF.  Now from Eq.~\eqref{Final_state_fermion}, the detection probabilities when each party gets exactly one particle where both Alice and Bob measure in external DoFs are given by 
\begin{equation}\label{path_path}
  \begin{tabular}{c | c c} 
  & $B$ : $R$ & $B$ : $U$  \\  
 \hline
 $A$ : $D$ \hspace{0.0005cm} & \hspace{0.0005cm} $\frac{1}{4}\text{cos}^2\phi$  & $\frac{1}{4}\text{sin}^2\phi$ \\ 
 $A$ : $L$ \hspace{0.0005cm} & \hspace{0.0005cm} $\frac{1}{4}\text{sin}^2\phi$  & $\frac{1}{4}\text{cos}^2\phi$ \\
\end{tabular},
\end{equation}
where $\phi=\left( \phi_{D} -\phi_{L} - \phi_{R}+ \phi_{U}\right) / 2$.

Now we assign dichotomic variables $+1$ and $-1$ for the detection events $\lbrace L,U \rbrace$ and $\lbrace D,R \rbrace$, respectively. Let $Pr_{mn}$ denote the probabilities of the coincidence events for Alice and Bob obtaining $m=\pm 1$ and $n=\pm 1$, respectively. The normalized expectation value is then given by
\begin{align} \label{Normal}
    E\left( \phi_{A},\phi_{B} \right)= &\dfrac{Pr_{++}-Pr_{-+}-Pr_{+-}+Pr_{--}}{Pr_{++}+Pr_{-+}+Pr_{+-}+Pr_{--}} \nonumber \\
    =& \text{cos} \left( \phi_{A} -\phi_{B} \right),
\end{align}
\noindent where $\phi_{A}=\left(\phi_{D}-\phi_{L}\right) $ and $\phi_{B}=\left( \phi_{U}-\phi_{R} \right)$. Now the CHSH~\cite{CHSH} inequality can be written as 
\begin{equation} \label{CHSH}
\vert E\left( \phi^{0}_{A},\phi^{0}_{B} \right) + E\left( \phi^{1}_{A},\phi^{0}_{B} \right)+ E\left( \phi^{0}_{A},\phi^{1}_{B} \right) - E\left( \phi^{1}_{A},\phi^{1}_{B} \right) \vert \leq 2,
\end{equation}
where the superscripts $0$ and $1$ stand for two detector settings for each particles. Now for $\phi^{0}_{A}=0$, $\phi^{1}_{A}=\pi$, $\phi^{0}_{B}=\frac{\pi}{4}$, and $\phi^{1}_{B}=-\frac{\pi}{4}$, Eq.~\eqref{CHSH} can be violated maximally by obtaining Tsirelson's bound $2\sqrt{2}$~\cite{Tsirelson}.

Now if Alice and Bob both measure	 in internal DoFs, then  the detection probabilities can be written as
\begin{equation}\label{spin_spin}
   \begin{tabular}{c | c c} 
  & $B$ : $\downarrow$ & $B$ : $\uparrow$  \\  
 \hline\
 $A$ : $\downarrow$  & \hspace{0.0005cm}  $\frac{1}{4}\text{sin}^2\phi$ \hspace{0.1cm} & $\frac{1}{4}\text{cos}^2\phi$\\ 
 \hspace{0.001cm} $A$ : $\uparrow$  & \hspace{0.0005cm}  $\frac{1}{4}\text{cos}^2\phi$ \hspace{0.1cm} & $\frac{1}{4}\text{sin}^2\phi$ \\
\end{tabular}.
\end{equation}
If Alice measures in the internal DoF and Bob measures in  the external DoF, then  the detection probabilities can be written as 
\begin{equation} \label{spin_path}
\begin{tabular}{c | c c} 
  & $B$ : $R$ & $B$ : $U$  \\  
 \hline
 $A$ : $\downarrow$  & \hspace{0.0005cm} $\frac{1}{4}\text{sin}^2\phi$ \hspace{0.1cm} & $\frac{1}{4}\text{cos}^2\phi$\\ 
 $A$ : $\uparrow$ & \hspace{0.0005cm} $\frac{1}{4}\text{cos}^2\phi$ \hspace{0.1cm} & $\frac{1}{4}\text{sin}^2\phi$ \\
\end{tabular}.
\end{equation}
If Alice measures in the external DoF and Bob measures in the internal DoF, then the detection probabilities can be written as 
\begin{equation} \label{path_spin}
\begin{tabular}{c | c c} 
  & $B$ : $\downarrow$ & $B$ : $\uparrow$  \\  
 \hline\
 $A$ : $D$  & \hspace{0.0005cm} $\frac{1}{4}\text{cos}^2\phi$ \hspace{0.1cm} & $\frac{1}{4}\text{sin}^2\phi$\\ 
 $A$ : $L$  & \hspace{0.0005cm} $\frac{1}{4}\text{sin}^2\phi$  \hspace{0.1cm} & $\frac{1}{4}\text{cos}^2\phi$ \\
\end{tabular}.
\end{equation}
 Now by applying similar analysis for Eqs.~\eqref{spin_spin},~\eqref{spin_path}, and~\eqref{path_spin}  as performed for Eqs.~\eqref{Normal} and~\eqref{CHSH}, one can show maximal violation of Bell's inequality. 

\subsection{Generalized Hyper-Hybrid entangled state} \label{Gen_boson_fermion}
Interestingly, following the approach by Yurke and Stolar~\cite{Y&S92PRA},
we can generalize the detection probabilities of hyper-hybrid entangled state for indistinguishable bosons and fermions into a single formulation as shown below. Let
\begin{equation}
\begin{aligned}
\phi_{1}=& \phi_{D}-\phi_{L}, \\ 
\phi_{2} =&
\begin{cases} 
      -\left( \phi_{R}-\phi_{U}\right)  & \text{for bosons} \\
      -\left( \phi_{R}-\phi_{U}\right)  + \frac{\pi}{2} & \text{for fermions} .
   \end{cases}
\end{aligned}
\end{equation}
The generalized detection probabilities of Eqs.~\eqref{path_path},~\eqref{spin_spin},~\eqref{spin_path}, and~\eqref{path_spin} are, respectively, given by 
\begin{eqnarray}
 \begin{tabular}{c | c c} 
  & $B$ : $R$ & $B$ : $U$  \\  
 \hline
 $A$ : $D$ & \hspace{0.1cm} $\frac{1}{4}\text{cos}^2(\phi_{1}-\phi_{2})$ \hspace{0.1cm} & $\frac{1}{4}\text{sin}^2(\phi_{1}-\phi_{2})$\\ 
 $A$ : $L$ & \hspace{0.1cm}  $\frac{1}{4}\text{sin}^2(\phi_{1}-\phi_{2})$ \hspace{0.1cm} & $\frac{1}{4}\text{cos}^2(\phi_{1}-\phi_{2})$ \\
\end{tabular},\\
 \begin{tabular}{c | c c} 
  & $B$ : $\downarrow$ & $B$ : $\uparrow$  \\  
 \hline
 $A$ : $\downarrow$ & \hspace{0.1cm} $\frac{1}{4}\text{sin}^2(\phi_{1}-\phi_{2})$ \hspace{0.1cm} & $\frac{1}{4}\text{cos}^2(\phi_{1}-\phi_{2})$\\ 
 $A$ : $\uparrow$ & \hspace{0.1cm} $\frac{1}{4}\text{cos}^2(\phi_{1}-\phi_{2})$ \hspace{0.1cm} & $\frac{1}{4}\text{sin}^2(\phi_{1}-\phi_{2})$ \\
\end{tabular},\\
 \begin{tabular}{c | c c} 
  & $B$ : $R$ & $B$ : $U$  \\  
 \hline
 $A$ : $\downarrow$ &\hspace{0.1cm} $\frac{1}{4}\text{sin}^2(\phi_{1}-\phi_{2})$ \hspace{0.1cm} & $\frac{1}{4}\text{cos}^2(\phi_{1}-\phi_{2})$\\ 
 $A$ : $\uparrow$ & \hspace{0.1cm} $\frac{1}{4}\text{cos}^2(\phi_{1}-\phi_{2})$ \hspace{0.1cm} & $\frac{1}{4}\text{sin}^2(\phi_{1}-\phi_{2})$ \\
\end{tabular},\\
 \begin{tabular}{c | c c} 
  & $B$ : $\downarrow$ & $B$ : $\uparrow$  \\  
 \hline
 $A$ : $D$ & \hspace{0.1cm} $\frac{1}{4}\text{cos}^2(\phi_{1}-\phi_{2})$ \hspace{0.1cm} & $\frac{1}{4}\text{sin}^2(\phi_{1}-\phi_{2})$\\ 
 $A$ : $L$ & \hspace{0.1cm} $\frac{1}{4}\text{sin}^2(\phi_{1}-\phi_{2})$ \hspace{0.1cm} & $\frac{1}{4}\text{cos}^2(\phi_{1}-\phi_{2})$ \\
\end{tabular}.
\end{eqnarray}

Computations, following Eqs.~\eqref{Normal} and~\eqref{CHSH}, lead to the maximum violation of Bell's inequality. 



\section{Does the scheme of Li \textit{et al.}~\cite{HHNL} work for distinguishable particles?} \label{DisHHES}
We are interested to see whether the circuit of Li \textit{et al.}~\cite[Fig. 2]{HHNL} as shown in Fig.~\ref{fig:Lietal} gives the same results for two distinguishable particles. Let us calculate the term in the first row and first column of Eq.~\eqref{path_path} for fermions. It says that the probability of Alice detecting a particle in detector $D$ and Bob detecting a particle in detector $R$ is given by
\begin{equation}
\left| \frac{1}{4} \left[  e^{i\left( \phi_{R}+ \phi_{L} \right) } + e^{i\left( \phi_{D}+ \phi_{U} \right) } \right] \right|^{2}=\frac{1}{4} \text{cos}^{2}\phi.
\end{equation}
If the particles are made distinguishable, this probability is calculated as
\begin{equation}
 \left| \frac{1}{4} e^{i\left( \phi_{R}+ \phi_{L} \right) } \right|^{2} + \left| \frac{1}{4} e^{i\left( \phi_{D}+ \phi_{U} \right) } \right|^{2} =\frac{1}{8}.
\end{equation}
As for other terms of Eq.~\eqref{path_path}, each term of Eqs~\eqref{spin_spin},~\eqref{spin_path}, and~\eqref{path_spin} reduces to $\frac{1}{8}$. From that, one can easily show that the right hand side of Eq.~\eqref{Normal} becomes zero. Thus the Bell violation is not possible by the CHSH test. Similar calculations for the bosons lead to the same conclusion. So, the circuit of~\cite{HHNL} would not work for distinguishable particles.

\section{Signaling using unit fidelity quantum teleportation and hyper-hybrid entangled state} \label{Sig_UFQT_HHES}
In this section we will prove out main theorem and also derive two corollaries from that theorem.
\begin{theorem} \label{Th1}
If quantum particles (either distinguishable or indistinguishable) can simultaneously produce and perform hyper hybrid entangled state and unit fidelity quantum teleportation respectively then using that cloning of any arbitrary quantum state is possible.
\end{theorem}


 It is well-known that unit fidelity quantum teleportation~\cite{Popescu94} for distinguishable particles is possible using BSM and LOCC. Here, we show that if hyper-hybrid entangled state for distinguishable particles could exist, then one could construct a universal quantum cloning machine (UQCM)~\cite{QC05,QC14} using unit fidelity quantum teleportation and hyper-hybrid entangled state, and further, use that UQCM to achieve signaling. Throughout this thesis, by signaling we mean faster-than-light or superluminal communication across spacelike separated regions.
\begin{proof} 
Now we give a details proof of the Theorem~\ref{Th1}.
\subsection{Description of the protocol} Our signaling protocol works in three phases, as follows.

 \begin{figure}[h!] 
\centering
\includegraphics[width=0.8\textwidth]{./Chap4/Alice_Bob.eps} 
\caption{The singlet state $\ket{\psi}_{A_{1}B_{1}}$ is shared between DoF 1 of Alice and that of Bob, whereas hyper-hybrid entangled state $\ket{\chi}_{PQ}$ is kept by Bob.}
\label{fig:Alice_Bob}
\end{figure}


\subsubsection{First phase: initial set-up.} 
Suppose there are four particles $A$, $B$, $P$, and $Q$ each having two DoFs $1$ and $2$. The particle $A$ is with Alice and the remaining three are with Bob, who is spacelike separated from Alice. The pair $\left\lbrace A,B \right\rbrace$ is in the singlet state in DoF $1$  denoted by $\ket{\psi}_{A_{1}B_{1}}$ and the pair $\left\lbrace P,Q \right\rbrace$ is in hyper-hybrid entangled state using both the DoFs $1$ and $2$ denoted by $\ket{\chi}_{PQ}$. To access the DoF $i$ of particle $X$, we use the notation $X_i$, where $X \in \{A, B, P, Q\}$ and $i \in \{1, 2\}$. The situation is depicted in Fig.~\ref{fig:Alice_Bob}. 
Note that $\ket{\psi}_{A_{1}B_{1}}$ can be expressed in any orthogonal basis. We have taken only $Z$ basis or computational basis $\left\lbrace \ket{0}, \ket{1}\right\rbrace$ and $X$ basis or Hadamard basis $\left\lbrace \ket{+}, \ket{-}\right\rbrace$ such that 
\medmuskip=2mu
\thinmuskip=2mu
\thickmuskip=2mu 
\begin{equation}
\begin{aligned}
   \ket{\psi}_{A_{1}B_{1}}&= \frac{1}{\sqrt{2}} \left( \ket{01}_{A_{1}B_{1}}-\ket{10}_{A_{1}B_{1}}\right)\\ & =  \frac{1}{\sqrt{2}} \left(\ket{+-}_{A_{1}B_{1}}-\ket{-+}_{A_{1}B_{1}}\right). 
\end{aligned}
\end{equation}
\medmuskip=2mu
\thinmuskip=2mu
\thickmuskip=2mu 
Alice wants to transfer binary information instantaneously to Bob. Before going apart, Alice and Bob agree on the following convention.
\begin{enumerate}
\item If Alice wants to send zero to Bob, then she would measure in $Z$ basis on the DoF 1 of her particle so that the state of the DoF 1 of the particle at Bob's side would be either $\ket{0}$ or $\ket{1}$. 
\item If Alice wants to send $1$ to Bob, then she would measure in $X$ basis on the DoF 1 of her particle so that the state of the DoF 1 of the particle at Bob's side would be either $\ket{+}$ or $\ket{-}$.
\end{enumerate}


\subsubsection{Second phase: cloning of any unknown state.} 
There are two steps of our proposed UQCM as follows.
\begin{enumerate}
\item Alice does measurement on DoF 1 of her particle $A$, i.e., $A_1$ in either $Z$ basis or $X$ basis. After this measurement, the state on DoF 1 of particle $B$, i.e., $B_1$ on Bob's side, is in an unknown state $\ket{\phi} \in \left\lbrace \ket{0}, \ket{1}, \ket{+}, \ket{-} \right\rbrace$ and it is  denoted  by $\ket{\phi}_{B_1}$. 
\item After Alice's measurement, Bob performs BSM on DoF 1 of particles $B$ and $P$,  i.e., on $B_1$ and $P_1$. 
This results in an output $k$ as one of the four possible Bell states (as seen in standard teleportation protocol~\cite{QT93}). Based on this output $k$, suitable unitary operations $U_{k}$ are applied on both the DoFs of $Q$, i.e., $Q_1$ and $Q_2$, where $U_{k} \in \left\lbrace \mathcal{I}, \sigma_{x}, \sigma_{y}, \sigma_{z}\right\rbrace $, $\mathcal{I}$ being the identity operation and $\sigma_{i}$'s $\left( i = x, y, z \right)$ the Pauli matrices.
As the first DoF of particle $P$, $P_1$ is maximally entangled with both the DoFs of $Q$, i.e., $Q_1$ and $Q_2$; thus, using BSM on DoFs $B_1$ and $P_1$ and suitable unitary operations on DoFs $Q_1$ and $Q_2$, the unknown state $\ket{\phi}$ on DoF ${B_1}$ is copied to both the DoFs $Q_1$ and $Q_2$. This part of the circuit, shown in Fig.~\ref{fig:NO_CLONING}, acts as a UQCM. 
\end{enumerate}

\begin{figure}[t!] 
\centering
\includegraphics[width=0.8\textwidth]{./Chap4/NO_CLONING.eps} 
\caption{Our proposed universal quantum cloning machine to demonstrate the impossibility of hyper-hybrid entangled state using distinguishable particles. Inputs to this cloning machine are the unknown quantum state $\ket{\phi}$ of DoF 1 of the particle $B$ (denoted by $\ket{\phi}_{B_{1}}$) and the hyper-hybrid entangled state $\ket{\chi}_{PQ}$, as shown in Fig.~\ref{fig:Alice_Bob}. More specifically, $\ket{\phi}_{B_{1}}$ is the state unknown to Bob generated on Bob's side after Alice does measurement on $A_1$ in either $Z$ basis or $X$ basis. After that, Bob performs BSM on $B_1$ and $P_1$, resulting in one of the four possible Bell states as output, denoted by $k$. Based on this output $k$, suitable unitary operations $U_{k}$ are applied on both the DoFs of $Q$, i.e., $Q_1$ and $Q_2$, where $U_{k} \in \left\lbrace \mathcal{I}, \sigma_{x}, \sigma_{y}, \sigma_{z}\right\rbrace $, $\mathcal{I}$ being the identity operation and $\sigma_{i}$'s $\left( i = x, y, z \right)$ the Pauli matrices. As a result, the unknown state $\ket{\phi}$ of $B_1$ is copied to both $Q_1$ and $Q_2$.}
\label{fig:NO_CLONING}
\end{figure}


\subsubsection{Third phase: decoding Alice's measurement basis.}
Now from the two copies of the unknown state $\ket{\phi}$ on the two DoFs of $Q$,  i.e., $\ket{\phi}_{Q_1}$ and $\ket{\phi}_{Q_2}$, Bob tries to discriminate the measurement bases of Alice, so that he can decode the information sent to him. For that, Bob measures both the DoFs of $Q$ in $Z$ basis, resulting in either $0$ or  $1$ in each of the DoFs. Now there are two possibilities.
\begin{enumerate}
\item If Alice has measured in $Z$ basis, then Bob's possible measurement results on the two DoFs of $Q$ are $\{00, 11\}$. 
\item On the other hand, if Alice has measured in $X$ basis, then Bob's possible measurement results on the two DoFs of $Q$ are $\{00, 01, 10, 11\}$.
\end{enumerate}
Suppose, Bob adopts the following strategy. Whenever his measurement results are all zero or all one (i.e., 00 or 11), then he concludes that Alice has sent a zero, and whenever he measures otherwise (i.e., 01 or 10) then he concludes that Alice has sent a 1.

\subsection{Computation of the signaling probability}
Let the random variables $X_A$ and $X_B$ denote the bit sent by Alice and the bit decoded by Bob, respectively. Hence, under the above strategy, Bob's success probability of decoding, which is also the probability of signaling, is given by
\begin{equation}
\begin{aligned}
P_{sig}  = & \Pr(X_A = 0 \wedge X_B = 0) + \Pr(X_A = 1 \wedge X_B = 1)\\
 = & \Pr(X_A = 0)\cdot\Pr(X_B = 0 \mid X_A = 0) \\
& + \Pr(X_A = 1)\cdot\Pr(X_B = 1 \mid X_A = 1)\\
 = & \frac{1}{2}\cdot 1 + \frac{1}{2}\cdot\frac{2}{4} = 0.75.
\end{aligned}
\end{equation}

To increase $P_{sig}$ further, Bob can use hyper-hybrid entangled state involving $N$ DoFs of $P$ and $Q$, with $N \geq 3$. Then he can make $N$ copies of the unknown state $\ket{\phi}$ into the DoFs of $Q$. Analogous, to the strategy above for the case $N=2$, here also if all the measurement results of Bob in the $N$ DoFs of $Q$ in $Z$ basis are the same, i.e., all-zero case or the all-one case, then Bob concludes that Alice has sent a zero; otherwise, he concludes that Alice has sent a 1. Thus, the above expression of $P_{sig}$ changes to
$$\frac{1}{2}\cdot 1 + \frac{1}{2}\cdot\frac{2^N-2}{2^N}.$$
In other words, 
\begin{equation}
\label{sigprob}
P_{sig}=1 - \frac{1}{2^N}.
\end{equation}   
By making $N$ larger and larger,  $P_{sig}$ can be made arbitrarily close to 1.
\end{proof}

\subsection{Experimental realization using optical circuits}
 For the experimental realization of the above protocol, we propose a circuit with DoF sorters, such as a	 spin sorter (SS), path sorter (PS), etc. (A spin sorter can be realized in an optical system using a polarizing beam splitter for sorting between the horizontal $\ket{H}$ and the vertical $\ket{V}$ polarizations of a photon. For an
alternative implementation in atomic systems using Raman process, one can see~\cite[Fig.~3]{HHNL}.)

\begin{figure}[t!] 
\centering
\includegraphics[width=0.8\textwidth]{./Chap4/SLS_N_2.eps} 
\caption{Bob's circuit for distinguishing between $Z$ and $X$ bases using two types of DoF sorters, i.e., a spin sorter (SS) and a path sorter (PS), and four detectors. Here the output of Fig.~\ref{fig:NO_CLONING} is used as an input in this circuit. Here, $\ket{\downarrow}$ and $\ket{\uparrow}$ denote the down- and the up-spin states of the particles, respectively. Further, $\ket{T}$ denotes the transverse mode and $\ket{R}$ denotes the reflected modes of a PS.}
\label{SLS_N_2}
\end{figure}

Suppose DoFs $1$ and $2$  are spin and path, respectively, with the two output states $\left\lbrace \ket{\downarrow}, \ket{\uparrow} \right\rbrace $ and $\left\lbrace \ket{T},\ket{R}\right\rbrace $. Here, $\ket{\downarrow}$ and $\ket{\uparrow}$ denote the down and the up spin states of the particles and $\ket{T}$ and $\ket{R}$ denote the transverse and the reflected modes of a PS, respectively. Without loss of generality, we take 
\begin{equation}
\begin{aligned}
\ket{0}=&\ket{\downarrow}=\ket{T}, \hspace{0.2cm} \ket{1}=\ket{\uparrow}=\ket{R}, \\  \ket{+}=&\frac{1}{\sqrt{2}}\left( \ket{\downarrow}+\ket{\uparrow}\right) =\frac{1}{\sqrt{2}}\left(\ket{T}+\ket{R}\right), \\
\ket{-}=&\frac{1}{\sqrt{2}}\left(\ket{\downarrow}-\ket{\uparrow}\right) =\frac{1}{\sqrt{2}}\left(\ket{T}-\ket{R}\right).
\end{aligned}
\end{equation}
The circuit, shown in Fig.~\ref{SLS_N_2}, takes as input particle $Q$ with DoFs $1$ and $2$, each having the cloned state $\ket{\phi}$ from the output of the circuit in Fig.~\ref{fig:NO_CLONING}. Bob places a path sorter $PS$ followed by two spin sorters $SS_{1}$ and $SS_{2}$ on two output modes of $PS$. Let $ D_{1}$ ($ D_{3}$) and $D_{2}$ ($ D_{4}$) be the detectors at the two output ports of $SS_{1}$ ($SS_{2}$).

If Alice measures in $Z$ basis, Bob detects the particles in $\left\lbrace D_{1},D_{4}\right\rbrace$ with unit probability. On the other hand, if she measures in $X$ basis, the particles would be detected in each of the detector sets $\left\lbrace D_{1},D_{4}\right\rbrace$ and $\left\lbrace D_{2},D_{3}\right\rbrace $ with a probability of 0.5. When Bob detects the particles in either $D_2$ or $D_3$, he instantaneously knows that the measurement basis of Alice is $X$. In this case, the signaling probability is 0.75, which can be obtained by putting $N=2$ in Eq.~\eqref{sigprob}.

For better signaling probability, one can use three DoFs $1$, $2$, and $3$, instead of two, in the joint state $\ket{\chi}_{PQ}$. The scheme for three DoFs is shown in Fig.~\ref{SLS_N_3}, where $S_{i}$ represents the sorter for DoF $i$, for $i \in \{1, 2, 3\}$. Now, if Alice  measures in $Z$ basis, Bob detects the particles in $\left\lbrace D_{1},D_{8}\right\rbrace $ with probability 1. But if she measures in $X$ basis, the particles would be detected in $\left\lbrace D_{1},D_{8}\right\rbrace $ with probability $\frac{2}{2^3}$ and in  $\left\lbrace D_{2}, \cdots , D_{7}\right\rbrace $ with probability $\frac{2^3 -2}{2^3}=0.75$. In this case, the signaling probability is 0.875, which can be obtained by putting $N=3$ in Eq.~\eqref{sigprob}.

We can generalize the above schematic as follows. Suppose, each of $P$ and $Q$ has $N$ DoFs (each degree having two eigenstates), numbered 1 to $N$, in hyper-hybrid entangled state $\ket{\chi}_{PQ}$. We also need to use $N$ corresponding types of DoF sorters. Now, if Alice measures in $Z$ basis, Bob detects the particles in $\left\lbrace D_{1},D_{2^N}\right\rbrace $ with probability 1. But if she measures in $X$ basis, the particles are detected in $\left\lbrace D_{1},D_{2^N}\right\rbrace $ with probability $\frac{2}{2^N}$ and in detectors  $\left\lbrace D_{2}, \cdots , D_{2^N-1}\right\rbrace $ with probability $\frac{2^N-2}{2^N}$. For $N$ DoFs, the signaling probability is given in Eq.~\eqref{sigprob}.

\begin{figure}[t!] 
\centering
\includegraphics[width=0.8\textwidth]{./Chap4/SLS_N_3.eps} 
\caption{Bob's circuit for distinguishing between $Z$ and $X$ bases using three types of DoF sorters, i.e., $S_1$, $S_2$, and $S_3$, and eight detectors. Here the output of Fig.~\ref{fig:NO_CLONING} is used as an input in this circuit.}
\label{SLS_N_3}
\end{figure}

\subsubsection{Increasing signaling probability without increasing the number of DoFs}
From Eq.~\eqref{sigprob}, it is clear that the signaling is possible only when $N$ is infinitely large. The existence of such a huge number of accessible DoFs may be questionable. Interestingly, we devise an alternative schematic that can drive the asymptotic success probability to 1 with only two DoFs but using many copies of the singlet state shared between Alice and Bob and the same number of copies of hyper-hybrid entangled state at Bob's disposal.

Suppose, Alice and Bob share $M$ copies of the singlet state \\
 $\left\lbrace  \ket{\psi^{(1)}}_{A_{1}B_{1}}, \ket{\psi^{(2)}}_{A_{1}B_{1}}, \cdots, \ket{\psi^{(M)}}_{A_{1}B_{1}}  \right\rbrace $ and Bob also has an equal number of copies of hyper-hybrid entangled states $ \left\lbrace \ket{\chi^{(1)}}_{PQ}, \ket{\chi^{(2)}}_{PQ}, \cdots, \ket{\chi^{(M)}}_{PQ}  \right\rbrace $ (a single copy of the singlet state and hyper-hybrid entangled state is shown in Fig.~\ref{fig:Alice_Bob}). Now the cloning can be performed in the following two steps.
\begin{enumerate}
\item  Alice performs measurement in her preferred basis on each DoF 1 of her $M$ particles so that on the DoF 1 of each of the $M$ particles on Bob's side, a copy of the unknown state $\ket{\phi}$ is obtained.
\item After that, Bob performs BSM on each of the $M$ pairs of $\left\lbrace B_1, P_1 \right\rbrace $ and suitable unitary operations so that the unknown state $\ket{\phi}$ is copied to each of the $M$ pairs of $\left\lbrace Q_1, Q_2 \right\rbrace $.
\end{enumerate}

Now Bob passes each of the $M$ copies of $Q$ as shown in Fig.~\ref{SLS_N_2} and adopts the following strategy. If Bob receives each of the $M$ particles in $D_{1}$ or $D_{4}$, then he concludes that Alice has measured in $Z$ basis. On the other hand, if Bob observes any one of the $M$ particles in $D_{2}$ or $D_{3}$, then he concludes that Alice has measured in $X$ basis. Under this strategy, Bob encounters a decoding error whenever Alice has measured in $X$ basis, but he receives all the $M$ particles in $D_{1}$ or $D_{4}$. 
In this case, the probability that a single particle is detected in the detector set $\left\lbrace D_{1},D_{4}\right\rbrace$ is $\frac{1}{2}$ and hence the probability that all the $M$ particles are detected in the above set is $\frac{1}{2^M}$. Hence, the corresponding success probability of signaling is given by 
\begin{equation}
    P_{sig}=1-\frac{1}{2^M},
\end{equation}
which also asymptotically goes to 1.


%The essence of the above discussion is that, in a world where special relativity holds barring signaling, HHES for distinguishable particles is not possible.
%\subsection{Logical representation and analysis}
Thus we have the following logical version of Theorem~\ref{Th1}
\begin{equation} \label{Cloning}
\text{HHES} \wedge \text{UFQT} \Rightarrow \text{Signaling}.
\end{equation}



\section{First no-go theorem: no hyper-hybrid entangled state for distinguishable particles} \label{NoHHES}
\begin{proof}

Unit fidelity quantum teleportation can be performed by distinguishable particles  ~\cite{QT93}. Thus if hyper-hybrid entangled state is also possible for distinguishable particles, it would lead to signaling as shown in Section~\ref{Sig_UFQT_HHES}. Thus a logical conclusion is that in a world where special relativity holds barring signaling, hyper-hybrid entangled state is not possible using distinguishable particles. Thus we can write this no-go theorem logically  as
\begin{equation} \label{no-HHES}
\text{No-signaling} \Rightarrow \text{no-HHES} \wedge \text{UFQT}.
\end{equation}
\end{proof}

\section{Second no-go theorem: no unit fidelity quantum teleportation for indistinguishable particles} \label{NoUFQT}

\begin{proof}

 Earlier, we have shown that signaling for distinguishable particles can be achieved using unit fidelity quantum teleportation and hyper-hybrid entangled state as black-boxes. unit fidelity quantum teleportation for distinguishable particles is already known~\cite{QT93}, and so we have concluded that hyper-hybrid entangled state for distinguishable particles must be an impossibility.

Using massive identical particles, Marzolino and Buchleitner~\cite{Ugo15} have shown that unit fidelity quantum teleportation is not possible using a finite and fixed number of indistinguishable particles, due to the particle number conservation superselection rule (SSR)~\cite{Wick52,SSR07}. Interestingly, several independent works~\cite{SSR07,Suskind67,Paterek11} have already established that this superselection rule can be bypassed. So, an obvious question is: whether it is possible to perform unit fidelity quantum teleportation for indistinguishable particles bypassing the superselection rule. This question is also answered in the negative in~\cite{Ugo15}. 

Very recently, for indistinguishable particles, Lo Franco and Compagno~\cite{LFC18} have achieved a quantum teleportation fidelity of $5/6$, overcoming the classical teleportation fidelity bound $2/3$~\cite{HHH99}. But they have not proved whether this value is optimal or whether unit fidelity can be achieved or not.

Systematic calculations show that our earlier scheme of quantum cloning and signaling (Figs.~\ref{fig:Alice_Bob} and Fig.~\ref{fig:NO_CLONING}) would still work, even if one replaces the unit fidelity quantum teleportation and hyper-hybrid entangled state tools for distinguishable particles with those of the indistinguishable ones (assuming that such tools exist). As signaling is not possible in quantum theory, we have concluded that hyper-hybrid entangled state for distinguishable particles is not possible. But, for indistinguishable particles, the creation of hyper-hybrid entangled state is possible~\cite{HHNL}. Thus, a logical conclusion is that, to prevent signaling, unit fidelity quantum teleportation must not be possible for indistinguishable particles. So, this no-go theorem can be represented logically as
\begin{equation}\label{no-UFQT}
\text{No-signaling} \Rightarrow \text{HHES} \wedge \text{no-UFQT}.
\end{equation}
\end{proof}


\section{Physical significance of the two no-go theorems} \label{Sepresult}
%\section{A separation result between distinguishable and indistinguishable particles} \label{Sepresult}
From the above two no-go results, we can establish a separation result between distinguishable and indistinguishable particles.  
Let $Q_{dis}$ and $Q_{indis}$ be the two sets consisting of quantum properties and applications of distinguishable and indistinguishable particles, respectively, as shown in Fig.~\ref{fig:Overall}.

 \begin{figure}[h!]
\centering
\includegraphics[width=0.8\textwidth]{./Chap4/Overall_pic.eps} 
\caption{The two sets $Q_{dis}$ (consisting of quantum properties and applications of distinguishable particles), $Q_{indis}$ (consisting of quantum properties and applications of indistinguishable particles), and their intersection (UFQT, HHES, and ES stand for unit fidelity quantum teleportation, hyper-hybrid entangled state, and entanglement swapping, respectively).} 
\label{fig:Overall}
\end{figure}

Several earlier works have attempted extending many results on one of these two sets to the other. For example, quantum teleportation was originally proposed for distinguishable particles~\cite{QT93,QTnat15}. But recent works~\cite{LFC18,Ugo15} have extended it for indistinguishable particles. Similarly, duality of entanglement as proposed in~\cite{Bose13} was thought to be a unique property of indistinguishable particles. But later its existence for distinguishable particle was shown in~\cite{M.Karczewski16}. Another unique property of quantum correlation is quantum coherence, which was proposed for distinguishable particles in~\cite{Baumgratz14} and later for indistinguishable particles in~\cite{Sperling17}. Einstein-Podolsky-Rosen steering~\cite{Schrodinger} was extended from distinguishable particles to a special class of indistinguishable particles called Bose-Einstein condensates~\cite{Fadel18}. Entanglement swapping, originally proposed for distinguishable particles in~\cite{ES93,Pan10,Pan19}, was also shown for indistinguishable particles in~\cite{LFCES19}.

To the best of our knowledge, there is no known quantum correlation or application that is unique for distinguishable particles only and does not hold for indistinguishable particles, and vice versa. In Section~\ref{NoHHES} of this paper, we have shown that hyper-hybrid entangled state is unique to the set $Q_{indis}$, and in Section~\ref{NoUFQT} we have established that unit fidelity quantum teleportation is unique to the set $Q_{dis}$. Thus, we demonstrate a clear separation between these two sets.



==> Cover/dedi.tex <==
\textbf{\textit{{\Large I dedicate this thesis to}
\\
{\LARGE My Parents}}}

==> Declaration/decla.tex <==
\begin{center}
\textbf{{\Large DECLARATION OF AUTHORSHIP}}
\end{center}
\medskip
I, \textbf{Soumya Das}, a student of Cryptology and Security Research Unit of the Ph.D. program of Indian Statistical Institute
Kolkata, hereby declare that the investigation presented in this thesis is based on my own work and, to the best of my knowledge, the materials contained in this thesis have not previously been published or written by any other person, nor it has been submitted as a whole or
as a part for any degree/diploma or any other academic award anywhere before.

\begin{flushleft}
\begin{figure}[h!]
\includegraphics[width=6cm]{./Declaration/soumyadas1.jpg} 
\end{figure}

Soumya Das \\
Cryptology and Security Research Unit \\
Indian Statistical Institute Kolkata \\
Kolkata 700108, West Bengal, India \\
\end{flushleft}
